Novel View Synthesis with View-Dependent Effects from a Single Image

In this paper, we firstly consider view-dependent effects into single image-based novel view synthesis (NVS) problems. For this, we propose to exploit the camera motion priors in NVS to model view-dependent appearance or effects (VDE) as the negative disparity in the scene. By recognizing specularities "follow" the camera motion, we infuse VDEs into the input images by aggregating input pixel colors along the negative depth region of the epipolar lines. Also, we propose a `relaxed volumetric rendering' approximation that allows computing the densities in a single pass, improving efficiency for NVS from single images. Our method can learn single-image NVS from image sequences only, which is a completely self-supervised learning method, for the first time requiring neither depth nor camera pose annotations. We present extensive experiment results and show that our proposed method can learn NVS with VDEs, outperforming the SOTA single-view NVS methods on the RealEstate10k and MannequinChallenge datasets.

==> Tables/table_nvsvdenet.tex <==
\begin{tabular}{lllcc}
\hline
Outputs & Layer descriptions & Inputs & Channels & Feature sizes\\  
\hline
$I_L$ & Input image & - & 3 & H$\times$W \\  
$P$ & Raw $(x,y)$ pixel locations & - & 2 & H$\times$W \\  
$F_{npe}$ & 1$\times$1Conv, ELU, 1$\times$1Conv, ELU & $P$ & 8 & H$\times$W \\  
Conv0 & 3$\times$3Conv, ELU, ResBlock & $I_L$ & 64 & H$\times$W \\  
Conv0$_{LR}$ & 3$\times$3Conv, ELU, ResBlock & $I^{(1/2)}_L$ & 64 & H/2$\times$W/2 \\  
Conv1 & 3$\times$3Conv(s2), ELU, ResBlock & Concat(Conv0, $F_{npe}$) & 128 & H/2$\times$W/2 \\  
Conv2 & 3$\times$3Conv(s2), ELU, ResBlock & Concat(Conv1, $F_{npe}$, Conv0$_{LR}$) & 256 & H/4$\times$W/4 \\  
Conv3 & 3$\times$3Conv(s2), ELU, ResBlock & Concat(Conv2, $F_{npe}$) & 256 & H/8$\times$W/8 \\  
Conv4 & 3$\times$3Conv(s2), ELU, ResBlock & Concat(Conv3, $F_{npe}$) & 256 & H/16$\times$W/16 \\
Conv5 & 3$\times$3Conv(s2), ELU, ResBlock & Concat(Conv4, $F_{npe}$) & 256 & H/32$\times$W/32 \\
Conv6 & 3$\times$3Conv(s2), ELU, ResBlock & Concat(Conv5, $F_{npe}$) & 256 & H/64$\times$W/64 \\
\hline
Dec6 & Nearest, 3$\times$3Conv, ELU & Conv6 & 128 & Conv5 \\  
iConv6 & 3$\times$3Conv, ELU & Concat(Dec6, Conv5) & 256 & Conv5 \\  
 
Dec5 & Nearest, 3$\times$3Conv, ELU & iConv6 & 128 & Conv4 \\  
iConv5 & 3$\times$3Conv, ELU & Concat(Dec5, Conv4) & 256 & Conv4 \\  

Dec4 & Nearest, 3$\times$3Conv, ELU & iConv5 & 128 & Conv3 \\  
iConv4 & 3$\times$3Conv, ELU & Concat(Dec4, Conv3) & 256 & Conv3 \\  

Dec3 & Nearest, 3$\times$3Conv, ELU & iConv4 & 128 & Conv2 \\  
iConv3 & 3$\times$3Conv, ELU & Concat(Dec3, Conv2) & 256 & Conv2 \\  

Dec2 & Nearest, 3$\times$3Conv, ELU & iConv3 & 128 & Conv1 \\  
iConv2 & 3$\times$3Conv, ELU & Concat(Dec2, Conv1) & 128 & Conv1 \\  

Dec1 & Nearest, 3$\times$3Conv, ELU & iConv2 & 64 & Conv0 \\ 

$D^L$ & 3$\times$3Conv & Concat(Dec1, Conv0) & $N$ & H$\times$W \\  

$VDE^L$ & 3$\times$3Conv & Concat(Dec1, Conv0) & $N_{vde}$ & H$\times$W \\  

\hline
\end{tabular}

==> Tables/table_posenet.tex <==
\begin{tabular}{lllcc}
\hline
Outputs & Layer descriptions & Inputs & Channels & Feature sizes\\  
\hline
Image Encoder \\
$I$ & Input image & - & 3 & H$\times$W \\  
Conv1 & 3$\times$3Conv(s2), ELU, ResBlock & $I$ & 32 & H/2$\times$W/2 \\  
Conv2 & 3$\times$3Conv(s2), ELU, ResBlock & Conv1 & 64 & H/4$\times$W/4 \\  
Conv3 & 3$\times$3Conv(s2), ELU, ResBlock & Conv2 & 128 & H/8$\times$W/8 \\  
Conv4 & 3$\times$3Conv(s2), ELU, ResBlock & Conv3 & 128 & H/16$\times$W/16 \\
\hline
Joint Encoder \\
$I_1, I^R_2$ & Concatenated rotation aligned pair & - & 6 & H$\times$W \\  
Conv1 & 3$\times$3Conv(s2), ELU, ResBlock & $I$ & 32 & H/2$\times$W/2 \\  
Conv2 & 3$\times$3Conv(s2), ELU, ResBlock & Conv1 & 64 & H/4$\times$W/4 \\  
Conv3 & 3$\times$3Conv(s2), ELU, ResBlock & Conv2 & 128 & H/8$\times$W/8 \\  
Conv4$_{joint}$ & 3$\times$3Conv(s2), ELU, ResBlock & Conv3 & 128 & H/16$\times$W/16 \\
\hline
Pose Estimator \\
Conv5 & 3$\times$3Conv(s2), ELU, ResBlock & Conv4$_1$, Conv4$_2$ & 128 & H/32$\times$W/32 \\
Conv6 & 3$\times$3Conv(s2), ELU, ResBlock & Conv5 & 256 & H/64$\times$W/64 \\
Conv7 & 1$\times$1Conv, ELU & Conv6 & 256 & H/64$\times$W/64 \\
$R_0, \bm{t}_0$ & 1$\times$1Conv, ELU & GAP(Conv7) & 6 & 1 \\
\hline
$\Delta$ Pose Estimator \\
Conv5 & 3$\times$3Conv(s2), ELU, ResBlock & Conv4$_{joint}$, Conv4$_1$, Conv4$_2$ & 128 & H/32$\times$W/32 \\
Conv6 & 3$\times$3Conv(s2), ELU, ResBlock & Conv5 & 256 & H/64$\times$W/64 \\
Conv7 & 1$\times$1Conv, ELU & Conv6 & 256 & H/64$\times$W/64 \\
$\Delta R, \Delta \bm{t}$ & 1$\times$1Conv, ELU & GAP(Conv7), $R_0, \bm{t}_0$ & 6 & 1 \\
\hline

$I_1$ & Input image & - & 3 & H$\times$W \\ 
$I_2$ & Input image (target view in NVS) & - & 3 & H$\times$W \\  

Conv4$_1$ & Image Encoder & $I_1$ & 128 & H/16$\times$W/16 \\ 
Conv4$_2$ & Image Encoder & $I_2$ & 128 & H/16$\times$W/16 \\ 

$R_0, \bm{t}_0$ & Pose Estimator & Conv4$_1$, Conv4$_2$ & 6 & 1 \\

$I^R_2$ & $I^R_2 = I(g(R_0))$ & $I_2$, $R_0$, & 3 & H$\times$W \\

Conv4$_{joint}$ & Joint Encoder & $I_1$, $I^R_2$ & 128 & H/16$\times$W/16 \\ 

$\Delta R, \Delta \bm{t}$ & $\Delta$ Pose Estimator & Conv4$_{joint}$, Conv4$_1$, Conv4$_2$, $R_0, \bm{t}_0$ & 6 & 1 \\

$R, \bm{t}$ & $R = R_0 + \Delta R, \bm{t} = \bm{t}_0 + \Delta \bm{t}$ & $R_0, \Delta R, \bm{t}_0, \Delta \bm{t}$ & 6 & 1 \\

\hline
\end{tabular}
